Shining Light into the Tunnel: Understanding and Classifying Network Traffic of Residential Proxies

Emerging in recent years, residential proxies (RESIPs) feature multiple unique characteristics when compared with traditional network proxies (e.g., commercial VPNs), particularly, the deployment in residential networks rather than data center networks, the worldwide distribution in tens of thousands of cities and ISPs, and the large scale of millions of exit nodes. All these factors allow RESIP users to effectively masquerade their traffic flows as ones from authentic residential users, which leads to the increasing adoption of RESIP services, especially in malicious online activities. However, regarding the (malicious) usage of RESIPs (i.e., what traffic is relayed by RESIPs), current understanding turns out to be insufficient. Particularly, previous works on RESIP traffic studied only the maliciousness of web traffic destinations and the suspicious patterns of visiting popular websites. Also, a general methodology is missing regarding capturing large-scale RESIP traffic and analyzing RESIP traffic for security risks. Furthermore, considering many RESIP nodes are found to be located in corporate networks and are deployed without proper authorization from device owners or network administrators, it is becoming increasingly necessary to detect and block RESIP traffic flows, which unfortunately is impeded by the scarcity of realistic RESIP traffic datasets and effective detection methodologies. To fill in these gaps, multiple novel tools have been designed and implemented in this study, which include a general framework to deploy RESIP nodes and collect RESIP traffic in a distributed manner, a RESIP traffic analyzer to efficiently process RESIP traffic logs and surface out suspicious traffic flows, and multiple machine learning based RESIP traffic classifiers to timely and accurately detect whether a given traffic flow is RESIP traffic or not.

==> 7_related_works.tex <==
\subject{Residential proxies}. 
A set of works focus on profiling the scale and distribution of residential proxies (RESIPs)~\cite{mi2019resident, DBLP:conf/ndss/MiTLLQ021,DBLP:conf/ccs/YangYMTGLZD22}. Particularly, Mi, et al.~\cite{mi2019resident} captured more than 6 million residential proxies during 2017 for 5 RESIP services, while Yang et al.~\cite{DBLP:conf/ccs/YangYMTGLZD22} moved forward to profile RESIPs in China along with over 4 million China RESIPs captured during 2021.
Besides, Chiapponi et al~\cite{DBLP:conf/icsoc/ChiapponiDTCT20} proposed several mathematical approaches to model the scale of RESIPs. 

% Upon the topic of residential proxies, a set of works focus on profiling the scale and distribution of residential proxies (RESIP)~\cite{mi2019resident, DBLP:conf/ndss/MiTLLQ021,DBLP:conf/ccs/YangYMTGLZD22}. Among these works, Mi, et al.~\cite{mi2019resident} captured more than 6 million residential proxies during 2017 for 5 RESIP services. This is achieved through sending HTTP probes through residential proxies toward web servers under the control of the researchers. Furthermore, Yang et al.~\cite{DBLP:conf/ccs/YangYMTGLZD22} moved forward to profile RESIPs in China along with over 4 million China RESIPs captured during 2021.
% As learned from these datasets, residential proxies are widely distributed and large-scale. Also, most residential proxies work in a backconnect mode wherein the relaying traffic will first be inter-mediated by one or more proxy gateways before existing from the residential proxies. 
% % However, as revealed in \cite{DBLP:conf/ccs/YangYMTGLZD22}, some China RESIP services offer direct RESIPs, which work like traditional web proxies and listen to network ports for incoming relaying traffic. 
% Besides, Chiapponi et al~\cite{DBLP:conf/icsoc/ChiapponiDTCT20} proposed two mathematical approaches to model the scale of REISPs. One is to abstract this task by a probabilistic drawing process with or without replacement, while the other is to design a fitting function to approximate the cumulative distribution of observed RESIP IPs across the measurement period.

Furthermore, several recruitment channels for RESIPs~\cite{upnproxy, mi2019resident, DBLP:conf/ndss/MiTLLQ021} have been revealed, e.g., the recruitment of potentially unwanted programs (PUPs)~\cite{mi2019resident}, and deploying RESIP nodes as 3rd-party SDKs of mobile apps~\cite{DBLP:conf/ndss/MiTLLQ021}. Besides, some studies also profiled the usage of RESIPs in malicious activities. Particularly, Mi, et al.~\cite{mi2019resident} found out that RESIPs had been abused to relay malicious traffic such as advertisement frauds and blackhat SEO. Compared to these previous studies, our work moves forward in several aspects. First of all, our BS nodes were deployed in multiple locations, which turns out to be capable of triggering more diverse relaying traffic. Our RESIP traffic dataset is much larger than previous ones with over 3 TBs in size and 92 millions in traffic flows. What is more important, we have conducted a much deeper analysis, which leads to the discovery of previously unknown malicious traffic categories.

% Furthermore, multiple studies~\cite{upnproxy, mi2019resident, DBLP:conf/ndss/MiTLLQ021} have investigated the recruitment channels of RESIPs. Particularly, a set of potentially unwanted programs (PUPs) on the Windows platform were found to serve as RESIP programs~\cite{mi2019resident}. Also, a signature-based Android proxy app scanner~\cite{DBLP:conf/ndss/MiTLLQ021} was built up, through which, hundreds of RESIP apps on the Android platform got identified. Given these RESIP programs, these studies further collected their traffic logs and profiled the usage and abuse of RESIPs. Through analyzing traffic logs of the 67 PUPs on the Windows platform,  Mi, et al.~\cite{mi2019resident} found out that RESIPS have been abused to relay malicious traffic such as advertisement frauds, blackhat SEO, and traffic towards malicious domain names. However, besides serving as a residential proxy, a PUP program may have other malicious functionalities, which may contribute to the resulting traffic logs. Therefore, it is unclear whether all the identified suspicious traffic flows were indeed relayed by the residential proxies. Similarly, given the hundreds of mobile proxy apps, the authors~\cite{DBLP:conf/ndss/MiTLLQ021} captured and analyzed their relaying traffic, from which, suspicious traffic categories got observed. However, the authors didn't mention the scale of the captured RESIP traffic, and their measurement infrastructure was only deployed only in the US. Compared to these previous studies, our work moves forward in several aspects in terms of collecting and understanding REISP traffic. First of all, our BS nodes were deployed in multiple locations, which turns out to be capable of triggering more diverse relaying traffic. Furthermore, regarding the scale of the relaying traffic, our dataset is much larger than previous ones with over 3TBs in size and 92 million in traffic flows. What is more important, we have conducted a much deeper analysis, which leads to the discovery of previously unknown malicious traffic categories.


% recruitment
% Some works also have made progress in terms of figuring out how residential proxies are recruited. As described in the white paper published in 2017, researchers at Akamai found that many NAT devices had vulnerabilities in their UPNP deployments, and such vulnerabilities allowed external attackers to do NAT entry injection and convert the NAT devies into web proxies. 
% Moving forward, Mi, et al.~\cite{DBLP:conf/ndss/MiTLLQ021} revealed the controversial recruitment of mobile devices as RESIPs and highlighted the privacy risks for mobile device users through a user study.

% Capturing and understanding relaying traffic

Considering the abuse of RESIPs in various malicious activities, multiple studies~\cite{DBLP:conf/ndss/MiTLLQ021,chiapponi_BADPASS_2022} explored possible features to identify RESIP traffic flows and designed various threshold-based methods to distinguish RESIP flows from benign ones. 
% Chiapponi et al.~\cite{chiapponi_BADPASS_2022} explored possible features to distinguish RESIP traffic flows, and found that a 
% relayed flow of RESIP can have a much higher gap between its TCP round trip time (RTT) and the respective TLS RTT. Therefore,  a threshold-based detection method was designed to capture this RTT gap and thus distinguish relayed flows from regular ones. However, this  methodology was only evaluated on a simulation dataset. 
Moving forward from these studies, our study has explored, for the first time,  the detection of both relayed flows and tunnel flows leveraging machine learning algorithms. Upon RESIP traffic flows that are both large-scaled and wild, our detection models turn out to be both effective and efficient. 

\subject{Security studies on network proxies}.
In addition to residential proxies, a long line of works have studied the security of other types of network proxies, particularly, VPNs~\cite{DBLP:conf/imc/IkramVSKP16, DBLP:conf/ndss/Donenfeld17, DBLP:conf/imc/KhanDVSKV18}, the Tor anonymity network~\cite{dingledine2004tor, murdoch2005low, overlier2006locating, murdoch2007sampled, bauer2007low}, and open web proxies~\cite{DBLP:conf/ndss/TsirantonakisII18,DBLP:conf/www/PerinoVS18}. Regarding the security of VPNs, Ikram et al~\cite{DBLP:conf/imc/IkramVSKP16} comprehensively evaluated Android VPN apps along with a set of concerning security issues discovered, e.g., the insecure tunneling technologies and TLS interception~\cite{DBLP:conf/imc/IkramVSKP16}. 
% Besides, Taha et al.~\cite{DBLP:conf/imc/KhanDVSKV18} moved the spotlight to commercial VPN services, and discovered that many VPN providers made false claims regarding the geographic diversity of their VPN servers. 
% Many VPN servers appear to be hosted in locations different from the ones advertised by the VPN providers. 
% To address the issues of existing VPN protocols and deployments, novel VPN protocols have been proposed, and one typical example is Wireguard~\cite{DBLP:conf/ndss/Donenfeld17}.

Besides, the Tor anonymity network~\cite{dingledine2004tor} has also attracted much research attention. Particularly, various attacks~\cite{murdoch2005low, overlier2006locating, murdoch2007sampled, bauer2007low, snader2008tune} have been proposed to either compromise or harden Tor's anonymity.  
% To defend against these attacks, multiple defense techniques have been proposed and evaluated, particularly, the opportunistic bandwidth measurement mechanism~\cite{snader2008tune}. 
Another line of works~\cite{DBLP:conf/ndss/JansenTJS14, jansen2019point} explored opportunities of denial of service attacks against the Tor relays, e.g., the Sniper attack~\cite{DBLP:conf/ndss/JansenTJS14}. 
Furthermore, as the Tor network gets increasingly adopted, many studies moved to profile the usage or even abuse of the Tor network. Specifically, McCoy et al.~\cite{mccoy2008shining} and Chaabane et al.~\cite{chaabane2010digging} profiled the usage of the Tor network along with malicious activities identified, e.g., hacking attempts and botnet communication. 
% In addition to the abuse from miscreants, traffic relayed by the Tor network was found to have suffered from service discrimination or blocking~\cite{singh2017characterizing}. To bypass Tor exit blocking, Zhang et al.~\cite{DBLP:conf/ccs/ZhangZS20} propose the use of short-lived proxies as alternative egress points for Tor traffic and they name such proxies as \textit{exit bridges}. 
The Tor network can also be used to hide network servers, which are named as onion services. Many studies have been conducted on onion services from various aspects, e.g.,  the illicit activities hosted on onion services~\cite{dolliver2015evaluating, dolliver2016characteristics, al2017classifying},  the fingerprintability of onion services~\cite{overdorf2017unique}, as well as attacks to de-anonymize the location of a hidden onion service~\cite{overlier2006locating, steinebach2019detection}.
% Murdoch et al.~\cite{murdoch2005low} propose a novel traffic analysis technique to effectively infer whether a given relay is used to relay an anonymous traffic stream. The authors observe that the traffic signatures of an anonymized traffic flow can be used to track the circuit of relays that the flow goes through. An attacker with only a partial view of the network can send probing traffic to a relay, and decide whether an anonymized flow has been routed through this relay by observing the resulting timing pattern of the probing traffic. Stepping forward, 
% Overlier et al.~\cite{overlier2006locating} demonstrate the feasibility of inferring the location of a hidden onion service leveraging a single malicious relay. Particularly, In the proposed attack, the attacker serves as both the initiator as well as a stable relay, which gives it the chance to serve as one of the intermediate relays between the hidden service and the rendezvous point. This gives the attacker the opportunity to learn the location of the hidden service. Furtheremore, as demonstrated in \cite{murdoch2007sampled}, Internet eXchanges(IXes) can be utilized to de-anonymize the Tor traffic.
% Then, to increase the probability of being selected for relaying traffic for a malicious relay, Kevin et al.~\cite{bauer2007low} propose and evaluate low-resource routing attacks wherein the malicous relay lies about its resources (e.g., claiming high bandwidth) so as to get selected by traffic initiators for relaying traffic. To defend agaist such kinds of low-resource attacks, an opportunistic bandwidth measurement mechanism is proposed in \cite{snader2008tune}. In the proposed mechanism, each relay keeps track of the peak bandwidth for each peer it has recently communicated with, and each traffic initiator will aggregate such bandwidth logs to get a global picture of the relays in terms of bandwidth. 
In addition, open (free) web proxies, as free proxies 
published on the web, have multiple security risks~\cite{DBLP:conf/ndss/TsirantonakisII18,DBLP:conf/www/PerinoVS18} identified. Particularly, Tsirantonakis et al.~\cite{DBLP:conf/ndss/TsirantonakisII18} studied the extent to which open HTTP proxies are involved in content modification for relayed traffic, and 5.15\% of the evaluated open HTTP proxies were found to have performed content modification or insertion. 
% Furthermore, Perino et al.~\cite{DBLP:conf/www/PerinoVS18} proposed  ProxyTorrent, a system that is designed to discover open web proxies, evaluate their performance, as well as detecting malicious activities performed by these proxies.
 

% \subject{Encrypted traffic classification}.  Compared with plaintext traffic classification , classifying encrypted network traffic incurs more challenges along with less robust features. Draper-Gil et al.\cite{draper2016characterization} explored classifying encrypted traffic flows using time-related features, e.g., the inter-packet arrival time. 
% Also, two classic machine learning algorithms, the decision tree and K-nearest neighbors (KNN), were evaluated, on the ISCXVPN2016 dataset comprising VPN (non-VPN) encrypted traffic flows of 7 categories. 
% Moving forward, Wang, et al.~\cite{wang2017end} demonstrated the effectiveness of one-dimensional CNN on encrypted traffic classification, along with higher performance results achieved on the ISCXVPN2016 dataset, when compared to \cite{draper2016characterization}. Wang, et al.~\cite{wang2017end} also found that 1D CNN outperforms 2D CNN by 2.51\% in accuracy, and features from bi-directional flows are better than that of one-direction flow. However, this study utilizes only the first 784 bytes of each traffic flow, and may not be able to classify stealthy encrypted traffic with key patterns hidden beyond the first 784 bytes. Furthermore, Wang, et al.~\cite{wang2017hast}  proposed and evaluated HAST-IDS for intrusion detection wherein packets are encoded using CNN while the resulting sequence of packet embeddings are merged through LSTM. HAST-IDS were trained and evaluated with state-of-the-art performance achieved, on two representative intrusion detection datasets, namely, DARPA1998 and ISCX2012.

\subject{Encrypted traffic classification}.  Compared with plaintext traffic classification, classifying encrypted network traffic incurs more challenges along with less robust features. Draper-Gil et al.\cite{draper2016characterization} explored time-related features, e.g., the inter-packet arrival time, while Wang, et al.~\cite{wang2017end, wang2017hast} demonstrated the effectiveness of one-dimensional CNN on encrypted traffic classification.
% Wang, et al.~\cite{wang2017end} also found that 1D CNN outperforms 2D CNN by 2.51\% in accuracy, and features from bi-directional flows are better than that of one-direction flow. However, this study utilizes only the first 784 bytes of each traffic flow, and may not be able to classify stealthy encrypted traffic with key patterns hidden beyond the first 784 bytes. 
% Furthermore, Wang, et al.~\cite{wang2017hast}  proposed and evaluated HAST-IDS for intrusion detection wherein packets are encoded using CNN while the resulting sequence of packet embeddings are merged through LSTM. HAST-IDS were trained and evaluated with state-of-the-art performance achieved, on two representative intrusion detection datasets, namely, DARPA1998 and ISCX2012.
Furthermore, He, et al.~\cite{he2020pert} adopted the spirit of word embedding, explored generic traffic representation, and proposed PERT. 
% And the masked language model proposed in BERT was adopted to do the pre-training. The authors also evaluated different strategies in terms of the number of packets to select, and the merging options for packet embedding vectors.
Moving forward, Lin, et al.~\cite{lin2022bert} proposed and evaluated Encrypted Traffic Bidirectional Encoder Representations from Transformer (ET-BERT). ET-BERT considers not only the inter-packet correlation but also the correlation between the incoming and outgoing flows of the same traffic session. Applying ET-BERT to multiple tasks of encrypted traffic classification has achieved state-of-the-art performance. 
Moving forward, Jorgensen et al.~\cite{jorgensen2022extensible} observed several limitations of the ISCXVPN2016 datasets (e.g.,  some VPN-labelled packets were found to have unencrypted payloads), and released a new traffic dataset under the name of \textit{VNAT}. 
% Along with this new traffic dataset is a machine learning framework which allows not only high prediction performance but also an interpretable score to flag novel traffic flows.

% Inspired by Bidirectional Encoder Representations from Transformers (BERT), He, et al. ~\cite{he2020pert} explored dynamic word embedding for encrypted network traffic and proposed PERT. To demonstrate the effectiveness of the pre-trained PERT, downstream supervised classification tasks on the ISCXVPN2016 datasets were carried out with state-of-the-art performance achieved, when compared to previous works~\cite{draper2016characterization, wang2017end, wang2017hast}. In PERT, each packet is converted into bi-gram tokens with each comprising two neighboring bytes. And the masked language model proposed in BERT was adopted to do the pre-training. The authors also evaluated different strategies in terms of the number of packets to select, and the merging options for packet embedding vectors. Moving forward, Lin, et al.~\cite{lin2022bert} proposed and evaluated Encrypted Traffic Bidirectional Encoder Representations from Transformer (ET-BERT). ET-BERT considers not only the inter-packet correlation of each traffic session (bi-directional flows) but also the correlation between the incoming and outgoing flows of the same traffic session. Applying ET-BERT to multiple encrypted traffic classification tasks has achieved state-of-the-art performance results. Moving forward, Jorgensen et al.~\cite{jorgensen2022extensible} observed several limitations of the widely used ISCXVPN2016 datasets. Particularly, some VPN-labelled  packets were found to have unencrypted payloads, and the assignment of  application categories is not consistent across PCAP files.   To address these limitations, a new dataset of VPN and non-VPN network traffic have been composed and released to the public under the name of \textit{VNAT}. Along with this new traffic dataset is a machine learning framework which allows not only high prediction performance but also an interpretable score to flag novel traffic flows.

% \xmi{TODO: Summarize this work publised in 2022: Extensible Machine Learning for Encrypted Network Traffic Application Labeling via Uncertainty Quantification}

==> ccs.tex <==
%% Rights management information.  This information is sent to you
%% when you complete the rights form.  These commands have SAMPLE
%% values in them; it is your responsibility as an author to replace
%% the commands and values with those provided to you when you
%% complete the rights form.

% \copyrightyear{2022} 
% \acmYear{2022} 
% \setcopyright{acmlicensed}\acmConference[CCS '22]{Proceedings of the 2022 ACM SIGSAC Conference on Computer and Communications Security}{November 7--11, 2022}{Los Angeles, CA, USA}
% \acmBooktitle{Proceedings of the 2022 ACM SIGSAC Conference on Computer and Communications Security (CCS '22), November 7--11, 2022, Los Angeles, CA, USA}
% \acmPrice{15.00}
% \acmDOI{10.1145/3548606.3559351}
% \acmISBN{978-1-4503-9450-5/22/11}

% \settopmatter{printacmref=true}

\setcopyright{none} % No copyright notice required for submissions
\acmConference[Anonymous Submission to ACM CCS 2023]{ACM Conference on Computer and Communications Security}{Due 4 May 2023}{Copenhagen, Denmark}
\acmConference{ACM Conference on Computer and Communications Security}{Due 4 May 2023}{Copenhagen, Denmark}
\acmYear{2023}

\settopmatter{printacmref=false, printccs=false, printfolios=true} % We want page numbers on submissions
\renewcommand\footnotetextcopyrightpermission[1]{} % removes footnote with conference information in first column
\pagestyle{plain} % removes running headersWe want page numbers on submissions


\author{Xianghang Mi}
\authornote{Corresponding author}
\orcid{0000-0002-8747-5601}
\affiliation{%
  \institution{University of Science and Technology of China}
}
\email{xmi@ustc.edu.cn}


==> deleted.tex <==
We also observed XX suspicious visits to XX government or education websites. For most HTTPs traffic, we cannot tell the specific activities since only the FQDN is revealed in TLS client hello message. However, several categories are still verified. 

- what actions/intentions can be extracted from visits to gov/edu websites? how do you decide these categories? For instance, how many flows were intended for login attempts? how many are for crawling sensitive datasets?

\subject{Account takeover}

- how do we decide a given traffic flow is account takeover?

 - http: signatures
 - https: login domains, 

- how many flows are observed to belong this category
   - how many are http, and how many are https
      - for http, what kind of passwords, accounts they have utilized xx
    - distribution across BS providers?
    - any burst pattern? 


Detail the imap email account login attempts
- attempts across imap domains?




\xmi{Any traffic to decide if a website is vulnerable? such as visiting a specific path?}

\subject{Suspicious traffic towards popular websites}. As detailed in \S\ref{sec:ecosystem}, XX\% of the relayed traffic are towards popular websites. However, as revealed in our control experiments, many traffic flows towards popular websites are of abnormal traffic patterns. 

\xmi{TODO: discuss on Dec 26 regarding the identified suspicious patterns and flows matching well with these patterns}
